MatchNorm: Learning-based Point Cloud Registration for 6D Object Pose Estimation in the Real World

In this work, we tackle the task of estimating the 6D pose of an object from point cloud data. While recent learning-based approaches to addressing this task have shown great success on synthetic datasets, we have observed them to fail in the presence of real-world data. We thus analyze the causes of these failures, which we trace back to the difference between the feature distributions of the source and target point clouds, and the sensitivity of the widely-used SVD-based loss function to the range of rotation between the two point clouds. We address the first challenge by introducing a new normalization strategy, Match Normalization, and the second via the use of a loss function based on the negative log likelihood of point correspondences. Our two contributions are general and can be applied to many existing learning-based 3D object registration frameworks, which we illustrate by implementing them in two of them, DCP and IDAM. Our experiments on the real-scene TUD-L, LINEMOD and Occluded-LINEMOD datasets evidence the benefits of our strategies. They allow for the first time learning-based 3D object registration methods to achieve meaningful results on real-world data. We therefore expect them to be key to the future development of point cloud registration methods.

==> fig/distribution_batch_0.tex <==
\begin{figure}[!ht]
    \centering
    % \includegraphics[width=\textwidth]{image/distribution_tudl.png}
    \includegraphics[width=\textwidth]{image/distribution_tudl_batch_0.png}
    \caption{\label{fig:db0} {\bf Feature distributions at different network layers with real-world data.} We show the distribution of the output of the different layer for different samples within one batch, with and without Match Normalization. Match Normalization consistently makes the source and target distributions much more similar.}

\end{figure}


==> fig/distribution_batch_1.tex <==
\begin{figure}[!ht]
    \centering
    % \includegraphics[width=\textwidth]{image/distribution_tudl.png}
    \includegraphics[width=\textwidth]{image/distribution_tudl_batch_1.png}
    \caption{\label{fig:db1} {\bf Feature distributions at different network layers with real-world data.} }

\end{figure}

==> fig/distribution_batch_2.tex <==
\begin{figure}[!ht]
    \centering
    % \includegraphics[width=\textwidth]{image/distribution_tudl.png}
    \includegraphics[width=\textwidth]{image/distribution_tudl_batch_2.png}
    \caption{\label{fig:db2} {\bf Feature distributions at different network layers with real-world data.} }
    \vspace{-2em}
\end{figure}

==> fig/distribution_batch_3.tex <==
\begin{figure}[!ht]
    \centering
    % \includegraphics[width=\textwidth]{image/distribution_tudl.png}
    \includegraphics[width=\textwidth]{image/distribution_tudl_batch_3.png}
    \caption{\label{fig:db3} {\bf Feature distributions at different network layers with real-world data.} }
    \vspace{-2em}
\end{figure}

==> fig/distribution_batch_4.tex <==
\begin{figure}[!ht]
    \centering
    % \includegraphics[width=\textwidth]{image/distribution_tudl.png}
    \includegraphics[width=\textwidth]{image/distribution_tudl_batch_4.png}
    \caption{\label{fig:db4} {\bf Feature distributions at different network layers with real-world data.} }
    \vspace{-2em}
\end{figure}

==> rebuttal_tex/table/norm_analysis.tex <==
\begin{table}[!h]
    \centering
    % \resizebox{\linewidth}{!}
    {\scriptsize
    \setlength{\tabcolsep}{0.7mm}{
    \begin{tabular}{l|cccccc|cccccc}
        \toprule
        & \multicolumn{6}{c|}{Rotation mAP} & \multicolumn{6}{c}{Translation mAP} \\
        Method & $5^{\circ}$ & $10^{\circ}$ & $15^{\circ}$ & $20^{\circ}$ & $25^{\circ}$ & $30^{\circ}$& $0.001$ & $0.005$ & $0.01$ & $0.05$ & $0.1$ & $0.5$ \\
        \midrule
        BN(SVD)    & 0.36 & 0.75 & 0.90 & 0.96 & 0.98 & 0.99 & 0.51 & 0.92 & 0.98 & 1.00 & 1.00 & 1.00 \\ % 1031 bnexp 45R svd bn Iter 10000
        BN(NLL pretrain+SVD) & 0.41 & 0.77 & 0.91 & 0.96 & 0.99 & 1.00 & 0.65 & 0.96 & 0.98 & 1.00 & 1.00 & 1.00 \\
        Identify  & 0.67 & 0.92 & 0.97 & 0.99 & 1.00 & 1.00 & 0.57 & 0.97 & 1.00 & 1.00 & 1.00 & 1.00 \\ % 0525_45R_nll_identify/epoch_16000.pth.tar
        BN   & 0.72 & 0.97 & 1.00 & 1.00 & 1.00 & 1.00 & 0.54 & 0.99 & 1.00 & 1.00 & 1.00 & 1.00 \\ % 1031 lossexp 45R nll Iter 10000
        BN+MN  & 0.84 & 0.97 & 0.99 & 1.00 & 1.00 & 1.00 & 0.51 & 0.89 & 0.98 & 1.00 & 1.00 & 1.00 \\ % 0525_45R_nll_bnmn/epoch_30000.pth.tar
        MN  & 0.85 & 0.97 & 0.99 & 1.00 & 1.00 & 1.00 & 0.51 & 0.91 & 0.99 & 1.00 & 1.00 & 1.00 \\ % 0525_45R_nll_mn_only/epoch_32000.pth.tar
        
        \bottomrule
    \end{tabular}
    }}
    \caption{{\bf Normalization and pre-trained model analysis.} The models are evaluated on the partial-to-partial registration task on ModelNet40 (clean), with $45^\circ$ rotation range. The one without marking SVD the backbone is DCP(V2) + NLL Loss, else is using SVD as loss function.
    }
    \label{tab:norm_analysis}
    % \vspace{-2em}
\end{table}

==> rebuttal_tex/table/running_time.tex <==
\begin{table}[!ht]
    \centering
    % \resizebox{\linewidth}{!}
    {\scriptsize
    \setlength{\tabcolsep}{0.5mm}{
    \begin{tabular}{l|ccccccccc}
    \toprule
    Method       & ICP & FGR & TEASER++ & Super4PCS  & Vidal-Sensors18 \\ 
    \midrule
    Time         & 12.1 & 32.1 & 213.5  & 3285.0  & 486.0 \\
    \midrule
    Method       & DCP(V2) & Ours+IDAM & Ours+DCP & Ours+DCP+ICP  & PPF-3D-ICP\\ 
    \midrule
    Time         & 14.2 & 17.3 & 18.8 & 26.7  & 143.0\\
    \bottomrule
    \end{tabular}
    }
    }
    \caption{Inference time in milliseconds.
    }
    \label{tab:running_time}
    \vspace{-1em}
\end{table}

==> rebuttal_tex/table/scale_analysis.tex <==
\begin{table}[!h]
    \centering
    {\scriptsize
    \setlength{\tabcolsep}{.8mm}{
    \begin{tabular}{l|ccc|ccc|cccc}
        \toprule
        & \multicolumn{3}{c|}{Rotation mAP} & \multicolumn{3}{c|}{Translation mAP} & \multicolumn{4}{c}{BOP Benchmark} \\
        Method & $5^{\circ}$ & $10^{\circ}$ & $20^{\circ}$ & $1cm$ & $2cm$ & $5cm$ & VSD & MSSD & MSPD & AR\\
        \midrule
        Input Scaling          & 0.55 & 0.66 & 0.78 & 0.50 & 0.74 & 0.95 & 0.540 & 0.750 & 0.751 & 0.680 \\
        Match Norm           & 0.70 & 0.81 & 0.87 & 0.71 & 0.86 & 0.97 & 0.700 & 0.853 & 0.852 & 0.801\\
        % Input Scaling          & 0.55 & 0.66 & 0.78 & 0.50 & 0.74 & 0.95 & 0.73 & 0.540 & 0.750 & 0.751 & 0.680 \\
        % scale+DCP+ICP      & 0.82 & 0.84 & 0.87 & 0.81 & 0.91 & 0.98 & 0.87 & 0.800 & 0.852 & 0.873 & 0.842 \\
        % Match Norm           & 0.70 & 0.81 & 0.87 & 0.71 & 0.86 & 0.97 & 0.85 & 0.700 & 0.853 & 0.852 & 0.801\\
        % Ours-DCP+ICP       & \textbf{0.91}& \textbf{0.92}& \textbf{0.93}& \textbf{0.86}& \textbf{0.95}& \textbf{0.99}& \textbf{0.93}& \textbf{0.859} & \textbf{0.914} & \textbf{0.935} & \textbf{0.903}\\
        \bottomrule
    \end{tabular}
    }}
    \caption{Input scaling vs Match Norm.}
    \label{tab:scale_analysis}
    \vspace{-1.25em}
\end{table}


==> rebuttal_tex/table/stability_analysis.tex <==
\begin{table}[!h]
    \centering
    % \resizebox{\linewidth}{!}
    {\scriptsize
    \setlength{\tabcolsep}{1.5mm}{
    \begin{tabular}{l|c|c}
    \toprule
    Method  & Crash Ratio & Crash Iteration                           \\
    \midrule
    DCP(V2) & 100\%       & 11, 2, 3, 5, 1, 2, 7, 4, 4, 1             \\
    PRNet   & 100\%       & 80, 7, 15, 33, 4, 4, 11, 15, 27, 8, 17, 2 \\
    RPMNet  & 100\%       & 114, 10, 9, 10, 10, 106, 11, 17, 52, 32, 1 \\
    \bottomrule
    \end{tabular}
    }
    }
    \caption{Stability analysis on the TUD-L dataset.
    }
    \label{tab:stability_analysis}
    \vspace{-2em}
\end{table}

==> rebuttal_tex/text.tex <==
We would like to thank the reviewers for their overall positive ratings, encouraging comments and helpful advice. \vspace{-1.3em}
\section*{To R1}
\vspace{-.5em}
\label{reason_1}
{\bf 1. Traditional methods.} The domain gap between the synthetic and real data affects the performance of learning based methods. Our method yields excellent results on TUD-L partly because the training set provided by the BOP benchmark contains real data. By contrast, the LINEMOD training set is synthetic, which degrades the performance. While our work constitutes an important step towards learning-based point-cloud registration, we acknowledge that some challenges remain open.  We will clarify this.
Note that traditional methods do not consistently yield good results. For example, while PPF-3D-ICP achieves the best score on LINEMOD, 
%with the AR value of 0.814, however 
its AR value on TUD-L is 0.776 (vs 0.91 for ours) on the~\href{https://bop.felk.cvut.cz/leaderboards/pose-estimation-bop19/tud-l/}{BOP Benchmark}. 
%In our opinion, the PPF estimator is optimized for curvature shape while not favor flat shape, it may account for its different behaviors on LINEMOD and TUD-L. 


%The biggest advantage of PPF-3D-ICP over learning algorithms is the generalisation ability of the algorithm. For the learning method, it's difficult to cross the gap between the synthetic data and real scene data. This is the case with the LINEMOD dataset, where the LINEMOD dataset only provides test data for real scenarios and no training data. Training is performed on the synthetic dataset.

%As for the Occluded-LINEMOD dataset, in addition to the reality gap, the occlusion is another challenging problem. The overlapping area of the two point cloud set is further reduced due to occlusion. This low overlapping problem is a well-known but still challenging issue. The existing outlier rejection layer (Sinkhorn layer) is effective for noise problems, but is still inadequate for this low overlapping ratio problem. This is a module that we think has a lot of room for improvement.

% 1. Two of the biggest challenges in the object 6D pose estimation task for the LINEMOD dataset are how to describe the objects and the noise and defects present in the real scene data. To the first challenge, both PPF-3D-ICP and our method use a global descriptor approach to describe objects. However, PPF demonstrates better robustness when dealing with noise and defects in real data. These noise and defects in real data are also challenging to the learning-based method, especially in the absence of training data from real scenes. This is the case with the LINEMOD dataset, which only provides real scene test data, but not training data. If the real scene data is provided the learning-based algorithm can performs well, as an evidence, TUD-L is similar to the LINEMOD dataset in terms of scene setting, but provides real scene training data. Perhaps in future work, the design of learning-based algorithms should give more thought to how an algorithm can be designed to make more efficient use of synthetic data so that it can perform better on real data.

% For the Occluded-LINEMOD dataset, the problem of occlusion is added to the problem of lack of real training data. In addition to the imaging principle of the camera itself, which makes the observed point cloud only part of the whole mesh model, occlusion further reduces the overlap between the two point clouds. As a result, all the algorithms produced varying degrees of performance degradation as shown in the Table3-5. To achieve better results on occlusion dataset like Occluded-LINEMOD for the learning-based algorithm, and the use of a simple outlier rejection mechanism may not be sufficient.

{\bf 2. Implementation details.} We will provide more implementation details in the final version and make our code publicly available upon acceptance of the paper.

{\bf 3 Ablation of the loss.} Thanks for the suggestion! We will evaluate both losses in the final version. In practise, SVD always crashes at the beginning of training when processing real data. With synthetic data, it cannot converge for the full rotation range and its performance on the $45^{\circ}$ range is not satisfying, as shown in Table 1 (main paper). The gradient instability in SVD back-propagation is the main cause and needs further studies. By contrast, the NLL loss is stable and outperforms SVD.
%for it imposes supervision directly on the score maps. 

% To be specific, we run the experiment ten times and it all crashed. They each crash at the iteration step of 12, 1, 36, 11, 10, 2, 30, 4, 2, 4, 8, 12, when the batch size is 32.
\vspace{-.7em}
\section*{To R3}
\vspace{-.5em}

% 1. \ZD{experiment:the gap between source and target distributions is coming due to outliers or partial observations. this part we need to pick the sample, provide the original sample with point cloud. The sample should contains the outliers and partial view. This part we could use some synthetic point cloud to highlight these issues.}

{\bf 1. Distribution gap.} 
Thanks! We will provide additional visualizations in the supplementary material.
Outliers lead to more dispersed feature distributions in the target domain.
%for diversified features. 
Partial observations yield more concentrated distributions as the network's features are more repetitive for the given fixed feature dimensionality.
%yields repetitive features in a fixed feature vector dimension when sampled partially.
\vspace{-.7em}

\input{rebuttal_tex/table/running_time}

{\bf 2. Inference time.} Table~\ref{tab:running_time} compares the inference times of different methods. Learning methods are generally faster than the traditional ones. We will include these numbers.

% and summarize the result in the table. As you can Table.~\ref{tab:running_time}. Ours-DCP yield comparable result with DCP(V2), while being faster than the traditional methods Vidal-Sensors18 and PPF-3D-ICP.

{\bf 3. Traditional methods.} As discussed in more detail in Answer 1 to R1, one difficulty for learning-based methods is the synthetic-to-real domain gap. While our work constitutes an important step towards learning-based point-cloud registration, we acknowledge that some challenges remain open. We will discuss this in the final version.

%Any methods to narrow the gap will enhance the performance. While PPF-3D-ICP behaves better on both LINEMOD and Occluded-LINEMOD, it does not work well on TUD-L as a result of its estimator design.

% In reponse to R1.1, we explained the reason why traditional method performs better than our on the LINEMOD dataset. 
% For the Occluded-LINEMOD dataset, the problem of occlusion is added to the problem of lack of real training data. 
% Occlusion further reduces the overlap between the two point clouds. 
% As a result, all the algorithms produced varying degrees of performance degradation as shown in the Table3-5. 
% To achieve satisfying results on occlusion dataset like Occluded-LINEMOD for the learning-based algorithm, the use of a simple outlier rejection mechanism may not be sufficient.

\input{rebuttal_tex/table/stability_analysis}

{\bf 4. SVD convergence.} We ran training 10 times for DCP(V2), PRNet, and RPMNet with random seeds on TUD-L. As shown in Table~\ref{tab:stability_analysis}, these algorithms always crashed, typically in the first few training iterations. 
\vspace{-.7em}
\section*{To R4}
\vspace{-.5em}

{\bf 1. Partial-to-partial.} In the literature, a partial-to-whole problem corresponds to the situation where every target point has a match in the source data (but not the reverse). This is not the case here because of noise and outliers.
%Every target point would find its correspondence in the source point set in ideal case. However, this assumption is violated by noises and outliers in the real scene data, in this case, the problem becomes a partial-to-partial problem.

%However, in the real-scene scenarios, there are two main factors existing violate this assumption which are the noise and outliers. The noise is a systemic error from the sensor, sometimes the depth from the sensor are discontinuous as a slice. This can produce large errors in describing a continuous smooth surface. The outlier can come from the edge of the object where it intersects with the background or other objects. These two factor lead to a result that some point in the target point set cannot find its corresponding point in the source point set. The end result is that only part of the target and source area can be overlapped. Thus we call this problem as a partial-to-partial problem. In our method, we use Sinkhorn layer with outlier label to label these point as outlier.

{\bf 2. SVD loss.} We have made significant efforts to make the SVD loss stable enough for us to benefit from its potential performance gain, but none of our attempts were successful.
%and see if it is the instability of itself to prevent us from benefiting its potential in performance, and we failed many times. 
This includes R4's suggestion of pre-training with the NLL loss and fine-tuning with the SVD one. On TUD-L, with Ours-DCP, the fine-tuning crashed at iteration 3, 1, 3, 24, 9, 2, 5, 7, 5, 3, respectively, in 10 trials. 
\vspace{-.6em}

% on the TUD-L dataset with the same experimental settings as the results shown in Table 2. 

% We tried this idea on the TUD-L dataset which experiment setting as same as in the Table 2. We use the model Ours-DCP as pre-trained model and then switch to SVD loss. However, we cannot finish the training process. It crash at the iteration 3, 1, 3, 24, 9, 2, 5, 7, 5, 3. 

% Additionally, we conducted experiments using synthetic data from the 45 degree interval, and train it till it converge.  Comparing with the model trained with SVD from scratch, the mAP increased by 5 percent over a 5 degree rotation interval for pre-trained model, as shown in the Table~\ref{tab:norm_analysis}. 

\input{rebuttal_tex/table/scale_analysis}
{\bf 3. Scaling each layer.} As shown in Table~\ref{tab:scale_analysis} for Ours-DCP on TUD-L, Match Normalization (scaling each layer) outperforms simple input scaling as it helps the network to regularize the features. We will include these results.

% We have tried this idea, as shown in the Table~\ref{tab:scale_analysis}, if only simply scale the input point cloud, the performance is worse than using Match Normalization.
% It is the affinity matrix that directly affects the construction of matches. 
% And the feature extracted by the network affects the affinity matrix. 
% In the experiment we found the mis-match of feature distribution between the source and target point cloud distribution. 

% We also tried the idea that only scaling the input point-cloud, 
% however, we found that is not enough. 
% Due to the existence of outlier in the target point cloud, the feature distribution mismatching will reappear in the subsequent layers. 
% In order to fix this problem, so we build the Match Normalization and put it within the network. 
% We also compared this idea with Match Normalization, 
% The results of match normalization are better than those of scaling only at the very beginning, and these results confirm our idea, as shown in the Table~\ref{tab:scale_analysis}


% \input{rebuttal_tex/table/norm_analysis}
% 4. \ZD{experiment:} The experiment is done. In Table.~\ref{tab:norm_analysis}
{\bf 4. Training efficiency.} Match Normalization (MN) does not affect the training efficiency as it adds no new learnable parameters. Without Batch Normalization (BN), MN converges in about the same number of iterations as with BN. 

{\bf 5. Model scale.} Thanks! We will state it in the paper.

\vspace{-.7em}
\section*{To R5}
\vspace{-.5em}

% 1. The role of the BN is to regularize feature output by the activation, however, it works individually, which therefore lead to the mismatch between source and target point cloud feature distributions. 
{\bf 1. BN vs MN.}
While Batch Normalization can help to prevent gradient explosion, it cannot address all 
%gradient-related 
issues, such as those due to SVD, or 
the feature distribution mismatch between the source and target point sets because BN acts on the individual sets. Match Normalization explicitly aims to address this latter issue. This is clearly stated in the introduction but we will aim to clarify the link with BN.

%1. Many factors may raise gradient problem, such as the back propagation of SVD; though Batch Normalization itself is not contributing to the problem, it cannot exert influences on other sources of gradient issues. The general issues affecting the stability of the gradient cannot be solely solved by modifying or changing backbones. 


% The proposed Match Normalization aims to address the mismatch feature distribution problem between the source and target point cloud. We find that the scaling factor is one of the main reasons for this, so we propose to share this key parameter between the two feature extractiion networks.

% The BN can prevent exploding gradient to some extent by regularize the data. However, the breakdown of the experiments mentioned in this paper was not caused by the normalization method. As state in the paper, the main reason is SVD loss. For the theoretical point of view, the problem at the place when calculating the gradient of the SVD. It's because of the eigenvalues of the matrix are too close to each other, thus leads to the problem of dividing the denominator by zero. The details can be found in the paper~\cite{Dang18}. To address this problem, we proposed to use NLL loss instead of SVD loss.

% Both of our idea shows effectiveness with different network architectures and widely used object 6D pose estimation datasets.

% 2. We conducted the comparison experiments on the widely used datasets and used the metric from the BOP benchmark which is also a commonly known benchmark. We use the script provided by the BOP benchmark to generate the results of these metrics, which can be found in the github repo \href{https://github.com/thodan/bop_toolkit}{BOP Toolkit}. For the SOTA method we either borrowed the result from the BOP benchmark, or we used the author released code to conduct the experiment ourself and to report the result. We'd also glad to know the ADD measure of which SOTA method is different from which paper reported result.

{\bf 2. SOTA performance.} 
We use the publicly released code to run others' algorithms and use the standard ADD metric. The differences mentioned by R5, although without clear pointer, are probably due to a misunderstanding; the performance of learning-based registration methods is typically reported on synthetic data, whereas we report results on real data. Existing methods indeed perform poorly in this setting, and we introduce solutions to remedy this.

%The NLL loss guarantees a stable training, and the proposed Match Normalization modifies the feature distribution of target domain to approaching that of source domain without adding complexity in training. This all improves the performance of learning methods on processing real scene data. We use the publicly released code to run others' algorithms and use the standard ADD metric with reference. I am open to check the differences of ADD you mentioned in other reports if you could kindly send to us. 




==> table/inference_time.tex <==
\begin{table}[!ht]
    \centering
    % \resizebox{\linewidth}{!}
    {\scriptsize
    \setlength{\tabcolsep}{2.0mm}{
    \begin{tabular}{l|ccccccccc}
    \toprule
    Method       & ICP & FGR & TEASER++ & Super4PCS  & Vidal-Sensors18 \\ 
    \midrule
    Time         & 12.1 & 32.1 & 213.5  & 3285.0  & 486.0 \\
    \midrule
    Method       & DCP(V2) & Ours+IDAM & Ours+DCP & Ours+DCP+ICP  & PPF-3D-ICP\\ 
    \midrule
    Time         & 14.2 & 17.3 & 18.8 & 26.7  & 143.0\\
    \bottomrule
    \end{tabular}
    }
    }
    \caption{Inference time in milliseconds.
    }
    \label{tab:running_time}
\end{table}
\vspace{-4em}

==> table/lm.tex <==
\begin{table*}[!htb]
    \centering
    {\scriptsize
    \setlength{\tabcolsep}{1.mm}{
    \begin{tabular}{l|cccccc|cccccc|c}
        \toprule
        & \multicolumn{6}{c|}{Rotation mAP} & \multicolumn{6}{c|}{Translation mAP} & \multicolumn{1}{c}{ADD}\\
        Method & $5^{\circ}$ & $10^{\circ}$ & $15^{\circ}$ & $20^{\circ}$ & $25^{\circ}$ & $30^{\circ}$& $0.5cm$ & $1cm$ & $2cm$ & $5cm$ & $10cm$ & $15cm$ & $0.1d$\\
        \midrule
        ICP         & 0.00 & 0.01 & 0.01 & 0.01 & 0.01 & 0.01 & 0.00 & 0.04 & 0.27 & 0.82 & 1.00 & 1.00 & 0.01 \\ % /home/hush/projects/teaser++/examples/teaser_python_fpfh_icp/0224icp_lm-test.csv
        FGR         & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.05 & 0.31 & 0.89 & 1.00 & 1.00 & 0.00 \\ % /home/hush/projects/teaser++/examples/teaser_python_fpfh_icp/0224fgr_lm-test.csv
        T++         & 0.01 & 0.03 & 0.04 & 0.05 & 0.07 & 0.08 & 0.00 & 0.03 & 0.21 & 0.73 & 0.95 & 0.99 & 0.03 \\ % /home/hush/projects/teaser++/examples/teaser_python_fpfh_icp/0224teaser_lm-test.csv
        Super4PCS   & 0.02 & 0.09 & 0.13 & 0.15 & 0.17 & 0.17 & 0.01 & 0.04 & 0.31 & 0.89 & 1.00 & 1.00 & 0.10 \\ % /home/hush/projects/bpnet-22-new/0228super4pcs_lm-test.csv
        DCP(v2)     & 0.00 & 0.00 & 0.01 & 0.01 & 0.02 & 0.02 & 0.00 & 0.05 & 0.24 & 0.83 & 1.00 & 1.00 & 0.00 \\ % /home/hush/projects/dcp/ckpt/0302_lm/models/model.best.t7
        %RPMNet      & 0.02 & 0.07 & 0.11 & 0.15 & 0.19 & 0.22 & 0.00 & 0.06 & 0.35 & 0.91 & 1.00 & 1.00 & 0.08 \\ % /home/hush/projects/RPMNet/logs/220301_115120_lmo/ckpt/model-best.pth
        % IDAM(GNN)   & 0.00 & 0.00 & 0.01 & 0.01 & 0.02 & 0.03 & 0.00 & 0.02 & 0.12 & 0.68 & 0.98 & 1.00 & 0.00 \\ % /home/hush/projects/idam/ckpt/0223_train_GNN_lmo/models/model.45.t7
        IDAM(FPFH)  & 0.00 & 0.01 & 0.01 & 0.03 & 0.04 & 0.06 & 0.00 & 0.03 & 0.16 & 0.67 & 0.95 & 0.99 & 0.01 \\ % /home/hush/projects/idam/ckpt/0304_train_FPFH_lm/models/model.4.t7
        IDAM(GNN-Norm) &0.00 & 0.00 & 0.01 & 0.02 & 0.03 & 0.05 & 0.01 & 0.04 & 0.16 & 0.72 & 0.98 & 1.00 & 0.01 \\ % /home/hush/projects/idam/ckpt/0301_train_GNNnorm_lmo/models/model.45.t7
        IDAM(DGCNN) & 0.00 & 0.02 & 0.04 & 0.07 & 0.09 & 0.11 & 0.01 & 0.05 & 0.25 & 0.84 & 0.99 & 1.00 & 0.03 \\ % /home/hush/projects/idam/ckpt/0228_train_DGCNN_lmo/models/model.45.t7
        Ours        & 0.10 & 0.27 & 0.40 & 0.49 & 0.55 & 0.59 & 0.07 & 0.26 & 0.60 & 0.95 & 1.00 & 1.00 & 0.37 \\
        Ours + ICP  & 0.43 & 0.59 & 0.64 & 0.67 & 0.70 & 0.71 & 0.09 & 0.49 & 0.83 & 0.97 & 1.00 & 1.00 & 0.60\\ % updated
        \bottomrule
    \end{tabular}
    }}
    \caption{Quantitative comparison of our method and the baselines on the \textbf{LineMod} real scene dataset.}
    \label{tab:lm}
    % \vspace{-1.25em}
\end{table*}

==> table/lm_bop.tex <==
\begin{table*}[!htb]
    \centering
    {\scriptsize
    \setlength{\tabcolsep}{2.2mm}{
    \begin{tabular}{l|cccc}
        \toprule
        & \multicolumn{4}{c}{BOP Benchmark}\\
        Method & vsd & mssd & mspd & average\_recall\\
        \midrule
        ICP    & 0.092 & 0.014 & 0.027 & 0.044 \\ % /home/hush/projects/teaser++/examples/teaser_python_fpfh_icp/0224icp_lm-test.csv
        FGR    & 0.068 & 0.000 & 0.010 & 0.026 \\ % /home/hush/projects/teaser++/examples/teaser_python_fpfh_icp/0224fgr_lm-test.csv
        T++    & 0.108 & 0.076 & 0.098 & 0.094 \\ % /home/hush/projects/teaser++/examples/teaser_python_fpfh_icp/0224teaser_lm-test.csv
        Super4PCS & 0.117 & 0.178 & 0.201 & 0.165 \\ % /home/hush/projects/bpnet-22-new/0228super4pcs_lm-test.csv
        DCP(v2)    & 0.057 & 0.025 & 0.049 & 0.044 \\ % /home/hush/projects/dcp/0305DCP_lm-test.csv
        %RPMNet     & 0.202 & 0.195 & 0.268 & 0.222 \\ %  /home/hush/projects/RPMNet/src/0302rpmnet_lm-test.csv 
        % IDAM(GNN)  & 0.037 & 0.035 & 0.046 & 0.039 \\ % /home/hush/projects/idam/0224idamGNN_lm-test.csv
        IDAM(FPFH) & 0.030 & 0.039 & 0.053 & 0.041 \\ % /home/hush/projects/idam/0225idamFPFH_lm-test.csv
        IDAM(GNN-Norm) & 0.046 & 0.055 & 0.066 & 0.056 \\ % /home/hush/projects/idam/0302idamGNNnorm_lm-test.csv
        IDAM(DGCNN) & 0.084 & 0.104 & 0.122 & 0.103 \\ % /home/hush/projects/idam/0302idamDGCNN_lm-test.csv
        % $\star$ PPF\_3D\_ICP & 0.679 & 0.819 & 0.817 & 0.779 \\
        $\star$ PPF\_3D\_ICP & 0.719 & 0.856 & 0.866 & 0.814 \\ 
        Ours         & 0.319 & 0.490 & 0.529 & 0.446 \\
        Ours + ICP   & 0.616 & 0.680 & 0.737 & 0.678 \\ % './ckpt/bpnet_real_detph_map_lm_MatchNorm_2/iter_30000.pth.tar'
        \bottomrule
    \end{tabular}
    }}
    \caption{Quantitative comparison of our method and the baselines on the \textbf{LineMod} real scene dataset.}
    \label{tab:lm_bop}
    % \vspace{-1.25em}
\end{table*}

==> table/lmo.tex <==
\begin{table*}[!htb]
    \centering
    {\scriptsize
    \setlength{\tabcolsep}{1.mm}{
    \begin{tabular}{l|cccccc|cccccc|c}
        \toprule
        & \multicolumn{6}{c|}{Rotation mAP} & \multicolumn{6}{c|}{Translation mAP} & \multicolumn{1}{c}{ADD}\\
        Method & $5^{\circ}$ & $10^{\circ}$ & $15^{\circ}$ & $20^{\circ}$ & $25^{\circ}$ & $30^{\circ}$& $0.5cm$ & $1cm$ & $2cm$ & $5cm$ & $10cm$ & $15cm$ & $0.1d$\\
        \midrule
        ICP         & 0.01 & 0.01 & 0.01 & 0.01 & 0.01 & 0.02 & 0.01 & 0.07 & 0.36 & 0.85 & 0.95 & 0.96 & 0.01 \\ % /home/hush/projects/teaser++/examples/teaser_python_fpfh_icp/0224icp_lmo-test.csv
        FGR         & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.01 & 0.08 & 0.43 & 0.85 & 0.96 & 0.96 & 0.00 \\ % /home/hush/projects/teaser++/examples/teaser_python_fpfh_icp/0224fgr_lmo-test.csv
        % T++         & 0.01 & 0.02 & 0.04 & 0.05 & 0.06 & 0.07 & 0.00 & 0.04 & 0.26 & 0.77 & 0.92 & 0.96 & 0.02 \\ % /home/hush/projects/teaser++/examples/teaser_python_fpfh_icp/0224teaser_lmo-test.csv
        Super4PCS   & 0.01 & 0.03 & 0.05 & 0.06 & 0.07 & 0.08 & 0.01 & 0.06 & 0.31 & 0.83 & 0.93 & 0.93 & 0.03 \\ % /home/hush/projects/bpnet-22-new/0228super4pcs_lmo-test.csv
        DCP(v2)     & 0.00 & 0.00 & 0.01 & 0.01 & 0.01 & 0.02 & 0.00 & 0.03 & 0.30 & 0.83 & 0.98 & 0.99 & 0.00 \\ % /home/hush/projects/dcp/ckpt/0302_lm/models/model.best.t7
        %RPMNet      & 0.02 & 0.04 & 0.08 & 0.12 & 0.16 & 0.20 & 0.02 & 0.08 & 0.34 & 0.87 & 0.98 & 0.99 & 0.04 \\ % /home/hush/projects/RPMNet/logs/220301_115120_lmo/ckpt/model-best.pth
        % IDAM(GNN)   & 0.00 & 0.01 & 0.01 & 0.02 & 0.03 & 0.03 & 0.00 & 0.02 & 0.14 & 0.70 & 0.95 & 0.96 & 0.00 \\ % /home/hush/projects/idam/ckpt/0223_train_GNN_lmo/models/model.45.t7
        IDAM(FPFH)  & 0.00 & 0.00 & 0.01 & 0.02 & 0.02 & 0.04 & 0.00 & 0.04 & 0.18 & 0.73 & 0.93 & 0.96 & 0.00 \\ % /home/hush/projects/idam/ckpt/0304_train_FPFH_lm/models/model.4.t7
        % IDAM(GNN-Norm) & 0.00 & 0.01 & 0.02 & 0.03 & 0.04 & 0.05 & 0.01 & 0.03 & 0.16 & 0.76 & 0.96 & 0.96 & 0.01 \\ % /home/hush/projects/idam/ckpt/0301_train_GNNnorm_lmo/models/model.45.t7
        IDAM(DGCNN) & 0.01 & 0.04 & 0.07 & 0.11 & 0.14 & 0.17 & 0.02 & 0.09 & 0.36 & 0.81 & 0.96 & 0.96 & 0.06 \\ % /home/hush/projects/idam/ckpt/0228_train_DGCNN_lmo/models/model.45.t7
        Ours        & 0.07 & 0.19 & 0.29 & 0.36 & 0.41 & 0.47 & 0.07 & 0.24 & 0.57 & 0.88 & 0.94 & 0.94 & 0.28 \\ 
        Ours + ICP  & 0.31 & 0.46 & 0.53 & 0.56 & 0.58 & 0.60 & 0.10 & 0.37 & 0.70 & 0.91 & 0.94 & 0.94 & 0.47 \\ % updated
        \bottomrule
    \end{tabular}
    }}
    \caption{Quantitative comparison of our method and the baselines on the \textbf{LineMod-O} real scene dataset.}
    \label{tab:lmo}
    % \vspace{-1.25em}
\end{table*}

==> table/lmo_bop.tex <==
\begin{table*}[!htb]
    \centering
    {\scriptsize
    \setlength{\tabcolsep}{2.2mm}{
    \begin{tabular}{l|cccc}
        \toprule
        & \multicolumn{4}{c}{BOP Benchmark}\\
        Method & vsd & mssd & mspd & average\_recall\\
        \midrule
        ICP    & 0.085 & 0.014 & 0.032 & 0.044 \\ % /home/hush/projects/teaser++/examples/teaser_python_fpfh_icp/0224icp_lmo-test.csv
        FGR    & 0.055 & 0.000 & 0.009 & 0.021 \\ % /home/hush/projects/teaser++/examples/teaser_python_fpfh_icp/0224fgr_lmo-test.csv
        T++    & 0.096 & 0.060 & 0.093 & 0.083 \\ % /home/hush/projects/teaser++/examples/teaser_python_fpfh_icp/0224teaser_lmo-test.csv
        Super4PCS & 0.054 & 0.072 & 0.113 & 0.080 \\ % /home/hush/projects/bpnet-22-new/0228super4pcs_lmo-test.csv
        DCP(v2)   & 0.055 & 0.018 & 0.059 & 0.044 \\ % /home/hush/projects/dcp/0305DCP_lmo-test.csv
        %RPMNet    & 0.154 & 0.160 & 0.238 & 0.184 \\ % /home/hush/projects/RPMNet/src/0302rpmnet_lmo-test.csv
        % IDAM(GNN) & 0.035 & 0.026 & 0.048 & 0.036 \\ % /home/hush/projects/idam/0224idamGNN_lmo-test.csv
        IDAM(FPFH) & 0.044 & 0.033 & 0.066 & 0.048 \\ % /home/hush/projects/idam/0305idamFPFH_lmo-test.csv
        IDAM(GNN-Norm) & 0.043 & 0.043 & 0.070 & 0.052 \\ % /home/hush/projects/idam/0302idamGNNnorm_lmo-test.csv
        IDAM(DGCNN) & 0.101 & 0.140 & 0.176 & 0.139 \\ % /home/hush/projects/idam/0302idamDGCNN_lmo-test.csv
        $\star$ Vidal-Sensors18 & 0.473 & 0.625 & 0.647 & 0.582 \\
        % $\star$ PPF\_3D\_ICP & 0.443 & 0.606 & 0.644 & 0.565 \\
        $\star$ PPF\_3D\_ICP & 0.523 & 0.669 & 0.716 & 0.636 \\
        Ours       & 0.263 & 0.384 & 0.450 & 0.365 \\
        Ours + ICP & 0.478 & 0.542 & 0.612 & 0.544 \\ % ./ckpt/bpnet_real_detph_map_lm_MatchNorm_2/iter_30000.pth.tar
        \bottomrule
    \end{tabular}
    }}
    \caption{Quantitative comparison of our method and the baselines on the \textbf{LineMod-O} real scene dataset.}
    \label{tab:lmo_bop}
    % \vspace{-1.25em}
\end{table*}

==> table/sup_lm_comb.tex <==
\begin{table*}[!t]
    \centering
    {\scriptsize
    \setlength{\tabcolsep}{1mm}{
    \begin{tabular}{l|ccc|ccc|c|cccc}
        \toprule
        & \multicolumn{3}{c|}{Rotation mAP} & \multicolumn{3}{c|}{Translation mAP} & \multicolumn{1}{c|}{ADD} & \multicolumn{4}{c}{BOP Benchmark} \\
        Method & $5^{\circ}$ & $10^{\circ}$ & $20^{\circ}$ & $1cm$ & $2cm$ & $5cm$ & $0.1d$ & VSD & MSSD & MSPD & AR\\
        \midrule
        ICP                 & 0.00 & 0.01 & 0.01 & 0.04 & 0.27 & 0.82 & 0.01 & 0.092 & 0.014 & 0.027 & 0.044 \\
        \rowcolor{tabgray}
        FGR(FPFH)           & 0.00 & 0.00 & 0.00 & 0.05 & 0.31 & 0.89 & 0.00 & 0.068 & 0.000 & 0.010 & 0.026 \\
        TEASER++(FPFH)      & 0.01 & 0.03 & 0.05 & 0.03 & 0.21 & 0.73 & 0.03 & 0.108 & 0.076 & 0.098 & 0.094 \\
        \rowcolor{tabgray}
        Super4PCS           & 0.02 & 0.09 & 0.15 & 0.04 & 0.31 & 0.89 & 0.10 & 0.117 & 0.178 & 0.201 & 0.165 \\
        DCP(v2)             & 0.00 & 0.00 & 0.01 & 0.05 & 0.24 & 0.83 & 0.00 & 0.057 & 0.025 & 0.049 & 0.044 \\ 
        % % IDAM(GNN)           & 0.02 & 0.06 & 0.11 & 0.02 & 0.09 & 0.49 & 0.07 & 0.076 & 0.110 & 0.105 & 0.097 \\
        \rowcolor{tabgray}
        IDAM(FPFH)          & 0.00 & 0.01 & 0.03 & 0.03 & 0.16 & 0.67 & 0.01 & 0.053 & 0.055 & 0.069 & 0.059 \\
        IDAM                & 0.00 & 0.01 & 0.05 & 0.03 & 0.16 & 0.71 & 0.02 & 0.050 & 0.070 & 0.081 & 0.067 \\ % IDAM(DGCNN) /home/hush/projects/idam/ckpt/0304_train_DGCNNdcp_lm/models/model.4.t7  /home/hush/projects/idam/0305idamDGCNNdcp_lm-test.csv
        \rowcolor{tabgray}
        $\star$PPF\_3D\_ICP & - & - & - & - & - & - & - & \textbf{0.719} & \textbf{0.856} & \textbf{0.866} & \textbf{0.814} \\ 
        $\star$Drost & - & - & - & - & - & - & - & 0.678 & 0.786 & 0.789 & 0.751 \\
        \rowcolor{tabgray}
        Ours-IDAM            & 0.01 & 0.07 & 0.15 & 0.13 & 0.38 & 0.87 & 0.11 & 0.148 & 0.194 & 0.209 & 0.184 \\ % IDAM(DGCNN+MN) /home/hush/projects/idam/ckpt/0304_train_DGCNN_lm/models/model.3.t7 /home/hush/projects/idam/0305idamDGCNN_lm-test.csv
        Ours-IDAM+ICP        & 0.15 & 0.23 & 0.27 & 0.25 & 0.54 & 0.91 & 0.23 & 0.352 & 0.311 & 0.345 & 0.336 \\ % IDAM(DGCNN+MN+ICP) /home/hush/projects/idam/ckpt/0304_train_DGCNN_lm/models/model.3.t7 /home/hush/projects/idam/0305idamDGCNNicp_lm-test.csv
        \rowcolor{tabgray}
        Ours-DCP            & 0.10 & 0.27 & 0.49 & 0.26 & 0.60 & 0.95 & 0.37 & 0.319 & 0.490 & 0.529 & 0.446 \\
        Ours-DCP+ICP        & \textbf{0.43} & \textbf{0.59} & \textbf{0.67} & \textbf{0.49} & \textbf{0.83} & \textbf{0.97} & \textbf{0.60} & 0.616 & 0.680 & 0.737 & 0.678 \\
        % Ours-DCP-Modelnet & 0.01 & 0.06 & 0.18 & 0.07 & 0.40 & 0.91 & 0.09 & 0.175 & 0.244 & 0.297 & 0.239 \\
        Ours-DCP+ICP-M & 0.25 & 0.35 & 0.42 & 0.34 & 0.66 & 0.93 & 0.36 & 0.449 & 0.446 & 0.499 & 0.465 \\  
        
        \bottomrule
    \end{tabular}
    }}
    \caption{Quantitative comparison of our method with previous work on the \textbf{LINEMOD} real scene dataset. PPF\_3D\_ICP~\cite{Drost10} and Drost (Drost-CVPR10-3D-Only)~\cite{Drost10} are traditional methods and represent the best depth-only performers from the BOP leaderboard.}
    \label{tab:lm_sup}
    \vspace{-1.25em}
\end{table*}


==> table/sup_lmo_comb.tex <==
\begin{table*}[!t]
    \centering
    {\scriptsize
    \setlength{\tabcolsep}{1mm}{
    \begin{tabular}{l|ccc|ccc|c|cccc}
        \toprule
        & \multicolumn{3}{c|}{Rotation mAP} & \multicolumn{3}{c|}{Translation mAP} & \multicolumn{1}{c|}{ADD} & \multicolumn{4}{c}{BOP Benchmark} \\
        Method & $5^{\circ}$ & $10^{\circ}$ & $20^{\circ}$ & $1cm$ & $2cm$ & $5cm$ & $0.1d$ & VSD & MSSD & MSPD & AR\\
        \midrule
        ICP                 & 0.01 & 0.01 & 0.01 & 0.07 & 0.36 & 0.85 & 0.01 & 0.085 & 0.014 & 0.032 & 0.044  \\
        \rowcolor{tabgray}
        FGR(FPFH)           & 0.00 & 0.00 & 0.00 & 0.08 & 0.43 & 0.85 & 0.00 & 0.055 & 0.000 & 0.009 & 0.021  \\
        TEASER++(FPFH)      & 0.01 & 0.02 & 0.05 & 0.04 & 0.26 & 0.77 & 0.02 & 0.096 & 0.060 & 0.093 & 0.083  \\
        \rowcolor{tabgray}
        Super4PCS           & 0.01 & 0.03 & 0.06 & 0.06 & 0.31 & 0.83 & 0.03 & 0.054 & 0.072 & 0.113 & 0.080 \\
        DCP(v2)             & 0.00 & 0.00 & 0.01 & 0.03 & 0.30 & 0.83 & 0.00 & 0.055 & 0.018 & 0.059 & 0.044 \\ 
        % \rowcolor{tabgray}
        % % IDAM(GNN)           & 0.02 & 0.06 & 0.11 & 0.02 & 0.09 & 0.49 & 0.07 & 0.076 & 0.110 & 0.105 & 0.097 \\
        \rowcolor{tabgray}
        IDAM(FPFH)          & 0.00 & 0.00 & 0.02 & 0.04 & 0.18 & 0.73 & 0.00 & 0.044 & 0.033 & 0.066 & 0.048 \\
        IDAM                & 0.00 & 0.02 & 0.06 & 0.07 & 0.26 & 0.76 & 0.02 & 0.063 & 0.088 & 0.119 & 0.090 \\ % IDAM(DGCNN) /home/hush/projects/idam/ckpt/0304_train_DGCNNdcp_lm/models/model.4.t7 /home/hush/projects/idam/0305idamDGCNNdcp_lmo-test.csv
        \rowcolor{tabgray}
        $\star$Vidal-Sensors18 & - & - & - & - & - & - & - & 0.473 & 0.625 & 0.647 & 0.582 \\
        $\star$PPF\_3D\_ICP & - & - & - & - & - & - & - & \textbf{0.523} & \textbf{0.669} & \textbf{0.716} & \textbf{0.636} \\
        \rowcolor{tabgray}
        Ours-IDAM            & 0.02 & 0.08 & 0.18 & 0.15 & 0.44 & 0.84 & 0.12 & 0.155 & 0.204 & 0.248 & 0.202 \\ % IDAM(DGCNN+MN) /home/hush/projects/idam/ckpt/0304_train_DGCNN_lm/models/model.3.t7 /home/hush/projects/idam/0305idamDGCNN_lmo-test.csv
        Ours-IDAM+ICP        & 0.15 & 0.22 & 0.32 & 0.23 & 0.58 & 0.88 & 0.25 & 0.349 & 0.320 & 0.374 & 0.348 \\ % IDAM(DGCNN+MN+ICP) /home/hush/projects/idam/ckpt/0304_train_DGCNN_lm/models/model.3.t7 /home/hush/projects/idam/0305idamDGCNNicp_lmo-test.csv
        \rowcolor{tabgray}
        Ours-DCP                & 0.07 & 0.19 & 0.36 & 0.24 & 0.57 & 0.88 & 0.28 & 0.263 & 0.384 & 0.450 & 0.365 \\
        Ours-DCP+ICP          & \textbf{0.31} & \textbf{0.46} & \textbf{0.56} & \textbf{0.37} & \textbf{0.70} & \textbf{0.91} & \textbf{0.47} & 0.478 & 0.542 & 0.612 & 0.544 \\
        % Ours-DCP-Modelnet & 0.01 & 0.04 & 0.14 & 0.09 & 0.39 & 0.84 & 0.06 & 0.138 & 0.186 & 0.256 & 0.193 \\
        Ours-DCP+ICP-M & 0.18 & 0.25 & 0.32 & 0.26 & 0.57 & 0.86 & 0.27 & 0.343 & 0.328 & 0.393 & 0.354 \\
        \bottomrule
    \end{tabular}
    }}
    \caption{Quantitative comparison of our method with previous work on the \textbf{Occluded-LINEMOD} real scene dataset. Vidal-Sensors18~\cite{Vidal18} and PPF\_3D\_ICP~\cite{Drost10} are traditional methods and represent the best depth-only performers from the BOP leaderboard.}
    \label{tab:lmo_sup}
    \vspace{-2.5em}
\end{table*}


==> table/sup_tudl_comb.tex <==
\begin{table*}[!ht]
    \centering
    {\scriptsize
    \setlength{\tabcolsep}{1.mm}{
    \begin{tabular}{l|ccc|ccc|c|cccc}
        \toprule
        & \multicolumn{3}{c|}{Rotation mAP} & \multicolumn{3}{c|}{Translation mAP} & \multicolumn{1}{c|}{ADD} & \multicolumn{4}{c}{BOP Benchmark} \\
        Method & $5^{\circ}$ & $10^{\circ}$ & $20^{\circ}$ & $1cm$ & $2cm$ & $5cm$ & $0.1d$ & VSD & MSSD & MSPD & AR\\
        \midrule
        ICP                 & 0.02 & 0.02 & 0.02 & 0.01 & 0.14 & 0.57 & 0.02 & 0.117 & 0.023 & 0.027 & 0.056 \\
        \rowcolor{tabgray}
        FGR(FPFH)           & 0.00 & 0.01 & 0.01 & 0.04 & 0.25 & 0.63 & 0.01 & 0.071 & 0.007 & 0.008 & 0.029 \\
        TEASER++(FPFH)      & 0.13 & 0.17 & 0.19 & 0.03 & 0.22 & 0.56 & 0.17 & 0.175 & 0.196 & 0.193 & 0.188 \\
        \rowcolor{tabgray}
        Super4PCS           & 0.30 & 0.50 & 0.56 & 0.05 & 0.40 & 0.92 & 0.54 & 0.265 & 0.500 & 0.488 & 0.418 \\
        DCP(v2)             & 0.00 & 0.01 & 0.02 & 0.02 & 0.07 & 0.55 & 0.01 & 0.0253 & 0.051 & 0.039 & 0.038 \\ 
        \rowcolor{tabgray}
        % IDAM(GNN)           & 0.02 & 0.06 & 0.11 & 0.02 & 0.09 & 0.49 & 0.07 & 0.076 & 0.110 & 0.105 & 0.097 \\
        IDAM(FPFH)          & 0.05 & 0.12 & 0.20 & 0.03 & 0.17 & 0.63 & 0.13 & 0.100 & 0.194 & 0.166 & 0.153 \\
        IDAM                & 0.03 & 0.05 & 0.10 & 0.02 & 0.08 & 0.49 & 0.05 & 0.067 & 0.108 & 0.099 & 0.091\\ % IDAM(DGCNN)
        \rowcolor{tabgray}
        $\star$Vidal-Sensors18 & - & - & - & - & - & - & - & 0.811 & 0.910 & 0.907 & 0.876 \\
        $\star$Drost & - & - & - & - & - & - & - & 0.809 & 0.875 & 0.872 & 0.852 \\
        \rowcolor{tabgray}
        Ours-IDAM           & 0.36 & 0.46 & 0.53 & 0.23 & 0.47 & 0.75 & 0.46 & 0.339 & 0.502 & 0.492 & 0.444\\ % IDAM(DGCNN+MN)
        Ours-IDAM+ICP       & 0.56 & 0.58 & 0.61 & 0.55 & 0.66 & 0.81 & 0.58 & 0.580 & 0.604 & 0.618 & 0.601\\ % IDAM(DGCNN+MN+ICP)
        \rowcolor{tabgray}
        Ours-DCP            & 0.70 & 0.81 & 0.87 & 0.71 & 0.86 & 0.97 & 0.85 & 0.700 & 0.853 & 0.852 & 0.801\\
        Ours-DCP+ICP       & \textbf{0.91}& \textbf{0.92}& \textbf{0.93}& \textbf{0.86}& \textbf{0.95}& \textbf{0.99}& \textbf{0.93}& \textbf{0.859} & \textbf{0.914} & \textbf{0.935} & \textbf{0.903}\\
        % Ours-DCP-Modelnet & 0.05 & 0.17 & 0.44 & 0.05 & 0.29 & 0.87 & 0.39 & 0.244 & 0.479 & 0.468 & 0.397 \\
        Ours-DCP+ICP-M & 0.62 & 0.66 & 0.72 & 0.60 & 0.73 & 0.89 & 0.70 & 0.666 & 0.706 & 0.725 & 0.699 \\ 
        \bottomrule
    \end{tabular}
    }}
    \caption{Quantitative comparison of our method with previous work on the \textbf{TUD-L} real scene dataset. The results for Vidal-Sensor18~\cite{Vidal18} and Drost (Drost-CVPR10-3D-Edges)~\cite{Drost10} were directly taken from the BOP leaderboard, and, in contrast with all the other results, were obtained without using a mask for the target point cloud. 
    `Ours-DCP+ICP-M' is the model which trained on the synthetic dataset ModelNet40. Our contributions not only allow existing learning-based methods to successfully register real-world data, but also keep their generalization ability to unseen objects.
    }
    \label{tab:tudl_sup}
    \vspace{-2.25em}
\end{table*}


==> table/tudl.tex <==
\begin{table*}[!htb]
    \centering
    {\scriptsize
    \setlength{\tabcolsep}{1.mm}{
    \begin{tabular}{l|cccccc|cccccc|c}
        \toprule
        & \multicolumn{6}{c|}{Rotation mAP} & \multicolumn{6}{c|}{Translation mAP} & \multicolumn{1}{c}{ADD}\\
        Method & $5^{\circ}$ & $10^{\circ}$ & $15^{\circ}$ & $20^{\circ}$ & $25^{\circ}$ & $30^{\circ}$& $0.5cm$ & $1cm$ & $2cm$ & $5cm$ & $10cm$ & $15cm$ & $0.1d$\\
        \midrule
        ICP         & 0.02 & 0.02 & 0.02 & 0.02 & 0.02 & 0.03 & 0.00 & 0.01 & 0.14 & 0.57 & 0.98 & 1.00 & 0.02 \\ % /home/hush/projects/teaser++/examples/teaser_python_fpfh_icp/0224icp_tudl-test.csv
        \rowcolor{tabgray}
        FGR(FPFH)         & 0.00 & 0.01 & 0.01 & 0.01 & 0.01 & 0.01 & 0.00 & 0.04 & 0.25 & 0.63 & 1.00 & 1.00 & 0.01 \\ % /home/hush/projects/teaser++/examples/teaser_python_fpfh_icp/0224fgr_tudl-test.csv
        TEASER++(FPFH)         & 0.13 & 0.17 & 0.18 & 0.19 & 0.20 & 0.21 & 0.00 & 0.03 & 0.22 & 0.56 & 0.90 & 0.99 & 0.17 \\ % /home/hush/projects/teaser++/examples/teaser_python_fpfh_icp/0224teaser_tudl-test.csv
        \rowcolor{tabgray}
        Super4PCS   & 0.30 & 0.50 & 0.55 & 0.56 & 0.57 & 0.57 & 0.00 & 0.05 & 0.40 & 0.92 & 0.98 & 1.00 & 0.54 \\ % /home/hush/projects/bpnet-22-new/0228super4pcs_tudl-test.csv
        DCP(v2)     & 0.00 & 0.01 & 0.01 & 0.02 & 0.03 & 0.06 & 0.00 & 0.02 & 0.07 & 0.55 & 0.88 & 0.99 & 0.01 \\ % /home/hush/projects/dcp/ckpt/0227_tudl/models/model.20.t7
        %RPMNet      & 0.83 & 0.92 & 0.94 & 0.95 & 0.96 & 0.96 & 0.45 & 0.86 & 0.96 & 0.99 & 1.00 & 1.00 & 0.95 \\ % /home/hush/projects/RPMNet/logs/220227_211443_tudl/ckpt/model-best.pth
        \rowcolor{tabgray}
        IDAM(GNN)   & 0.02 & 0.06 & 0.08 & 0.11 & 0.12 & 0.14 & 0.00 & 0.02 & 0.09 & 0.49 & 0.86 & 0.98 & 0.07 \\ % /home/hush/projects/idam/ckpt/0223_train_GNN_tudl/models/model.45.t7
        IDAM(FPFH)  & 0.05 & 0.12 & 0.16 & 0.20 & 0.22 & 0.25 & 0.00 & 0.03 & 0.17 & 0.63 & 0.96 & 1.00 & 0.13 \\ % /home/hush/projects/idam/ckpt/0224_train_FPFH_tudl/models/model.45.t7
        % IDAM(GNN-Norm) & 0.04 & 0.07 & 0.11 & 0.13 & 0.16 & 0.19 & 0.00 & 0.04 & 0.16 & 0.50 & 0.81 & 0.98 & 0.10 \\ % /home/hush/projects/idam/ckpt/0301_train_GNNnorm_tudl/models/model.45.t7
        \rowcolor{tabgray}
        IDAM(DGCNN) & 0.03 & 0.05 & 0.08 & 0.10 & 0.12 & 0.13 & 0.00 & 0.02 & 0.08 & 0.49 & 0.91 & 1.00 & 0.05 \\ % /home/hush/projects/idam/ckpt/0302_train_DGCNNdcp_tudl/models/model.45.t7
        IDAM(DGCNN+MN) & 0.36 & 0.46 & 0.50 & 0.53 & 0.55 & 0.57 & 0.06 & 0.23 & 0.47 & 0.75 & 0.94 & 0.99 & 0.46 \\ % /home/hush/projects/idam/ckpt/0228_train_DGCNN_tudl/models/model.45.t7
        \rowcolor{tabgray}
        IDAM(DGCNN+MN+ICP) & 0.56 & 0.58 & 0.59 & 0.61 & 0.62 & 0.63 & 0.04 & 0.55 & 0.66 & 0.81 & 0.95 & 1.00 & 0.58 \\ %
        Ours        & 0.70 & 0.81 & 0.84 & 0.87 & 0.89 & 0.90 & 0.50 & 0.71 & 0.86 & 0.97 & 1.00 & 1.00 & 0.85 \\
        \rowcolor{tabgray}
        Ours + ICP  & 0.91 & 0.92 & 0.93 & 0.93 & 0.93 & 0.94 & 0.04 & 0.86 & 0.95 & 0.99 & 1.00 & 1.00 & 0.93 \\ % ckpt/bpnet_real_detph_map_tudl_MatchNorm_2/iter_20000.pth.tar
        \bottomrule
    \end{tabular}
    }}
    \caption{Quantitative comparison of our method and the baselines on the \textbf{TUDL} real scene dataset.}
    \label{tab:tudl}
    % \vspace{-1.25em}
\end{table*}

==> table/tudl_bop.tex <==
\begin{table*}[!htb]
    \centering
    {\scriptsize
    \setlength{\tabcolsep}{2.2mm}{
    \begin{tabular}{l|cccc}
        \toprule
        & \multicolumn{4}{c}{TUD-L Dataset}\\
        Method & vsd & mssd & mspd & average\_recall\\
        \midrule
        ICP    & 0.117 & 0.023 & 0.027 & 0.056 \\ % /home/hush/projects/teaser++/examples/teaser_python_fpfh_icp/0224icp_tudl-test.csv
        FGR    & 0.071 & 0.007 & 0.008 & 0.029 \\ % /home/hush/projects/teaser++/examples/teaser_python_fpfh_icp/0224fgr_tudl-test.csv
        T++    & 0.175 & 0.196 & 0.193 & 0.188 \\ % /home/hush/projects/teaser++/examples/teaser_python_fpfh_icp/0224teaser_tudl-test.csv
        Super4PCS & 0.265 & 0.500 & 0.488 & 0.418 \\ % /home/hush/projects/bpnet-22-new/0228super4pcs_tudl-test.csv
        DCP(v2)   & 0.0253 & 0.051 & 0.039 & 0.038 \\ % /home/hush/projects/dcp/0302DCP_tudl-test.csv
        %RPMNet    & 0.784 & 0.924 & 0.923 & 0.877 \\ % /home/hush/projects/RPMNet/src/0301rpmnet_tudl-test.csv
        IDAM(GNN) & 0.076 & 0.110 & 0.105 & 0.097 \\ % /home/hush/projects/idam/0224idamGNN_tudl-test.csv
        IDAM(FPFH) & 0.100 & 0.194 & 0.166 & 0.153 \\ % /home/hush/projects/idam/0225idamFPFH_tudl-test.csv
        % IDAM(GNN-Norm) & 0.090 & 0.149 & 0.147 & 0.128 \\ % /home/hush/projects/idam/0302idamGNNnorm_tudl-test.csv
        IDAM(DGCNN) & 0.067 & 0.108 & 0.099 & 0.091 \\ % /home/hush/projects/idam/0302idamDGCNNdcp_tudl-test.csv
        IDAM(DGCNN+MN) & 0.339 & 0.502 & 0.492 & 0.444 \\ % /home/hush/projects/idam/0302idamDGCNN_tudl-test.csv
        IDAM(DGCNN+MN+ICP) & 0.580 & 0.604 & 0.618 & 0.601 \\ % 
        $\star$ Vidal-Sensors18 & 0.811 & 0.910 & 0.907 & 0.876 \\
        Ours         & 0.700 & 0.853 & 0.852 & 0.801 \\
        Ours + ICP   & 0.859 & 0.914 & 0.935 & 0.903 \\ % ./ckpt/bpnet_real_detph_map_tudl_MatchNorm_2/iter_20000.pth.tar
        
        \bottomrule
    \end{tabular}
    }}
    \caption{Quantitative comparison of our method and the baselines on the \textbf{TUD-L} real scene dataset.}
    \label{tab:tudl_bop}
    % \vspace{-1.25em}
\end{table*}

==> tex/baseline.tex <==
\input{table/baseline_result}

\section{Baseline Model}

We choose DCP(v2) to be our baseline model not just for its simplicity, but also for it provides a pipeline includes modern techniques and will be used for comparison. In the following section, we're going to reveal the full potential of the DCP method by changing a small amount but necessary component.

Since the original DCP method was designed to estimate the relative transformation between two fully observed pointcloud, it means the original DCP neither can handle the partial-to-partial pointcloud matching nor the self-occluded object pose estimation task. However, in the following section, we're going to show with the changes of three most crucial components, the DCP will first gain the power to handle wide rotation range, then able to handle the partial-to-partial pointcloud registration well and finally able to handle the self-occluded object pose estimation task even evaluated on the real scene data without any fine-tuning.

% \subsection{Baseline Method}

% We use DCP(v2) as our baseline method, but with few changes:

% \paragraph{1. input reduce mean.}
% Since the target pointcloud could be far from the camera then has a large magnitude of the value in the xyz. Here we reduce the mean on each axis to move the target pointcloud in a $[-1,1]$ cube. This move could be consider as normalization on the translation axis. After the estimation of the translation we add back the reduced mean. Since this is a small but crutial point we make it as the default setting. 

% \paragraph{2. remove the moving mean and var in the batch normalization.}
% In practice we found this achieve better performance, thus we keep this part as the default setting.

% \paragraph{3. optimizer change to be adam without scheduler.}
% The original DCP using a scheduler to control the learning rate, however, we found this part affect little on the performance. In order to keep the simplicity, we using the Adam with a fixed learning rate.

\subsection{Baseline Result}

Here we list three experiments each corresponding to different task. To be specific, the first one is the full object pointcloud registration task, the second one is the partial-to-partial pointcloud registration task, the last one is the real scene self-occluded object pose estimation task.

The result are summarize in the table~\ref{tab:baseline_result}


% ------------------------------------------------------------------------



% \input{fig/visible_surface}
% \input{fig/pipeline_compare}

% \subsection{Preliminary knowledge}

% Before we introduce our proposed method, here we review the widely used non-viewpoint rendering augmentation first. As done by e.g. PointnetLK DCP, which were designed to work under the unrealistic assumption that both point sets are fully observed, even at the test time, follow-up works focused on the more practical partial-to-partial registration scenario PRNet, RPMNet. Nevertheless, these techniques still assume the observations to depict a point-cloud in full 3D. To be specific, they take the fully observed 3D mesh model, sampling from the mesh model and then using two plane to slice the pointcloud into two pieces which have overlapped area. They called this kind of task to be partial-to-partial pointcloud matching. At first glance, the real scene case seems like just the sub task of this partial-to-partial pointcloud matching. But there are several things need to be noticed.

% 1. The object in the partial-to-partial pointcloud matching can be see through the inner structure, but in the self-occluded case is not. Some mesh model contains the inner structure, for example, a car with seats inside. If the seat can be observed, the partial-to-partial matching will have more matching point in the overlapping area, but these seats' pointcloud cannot be observed by the depth sensor, thus cannot find the corresponding point in the target pointcloud. Thus making the self-occluded task harder.

% 2. The noise in the partial-to-partial pointcloud matching is only Gaussian noise, but in the self-occluded case is not. In the self-occluded case, the mis-alignment of two point can be cause by the discrete sampling of the depth map. This kind of noise is cause by the imaging principle of camera, even create by the rendering also can not be avoid. Thus the error is system error, there is no guarantee that model trained with Gaussian noise can work on self-occluded task.

% 3. The partial-to-partial pointcloud matching's overlapping can be controled, but the self-occluded cannot. In the real scene scenario, if a guitar be observed from the front the overlapping area with the mesh model is close to 50\%. However, if it's been observed from the right-side, it looks like a slender rectangle. In this case the overlapping area is below 10\%. Thus make the self-occluded task harder.

% % 4. The partial-to-partial task slices the object's pointcloud making \textbf{all} the training and testing object asymmetrical, which reduced the difficulty. However, slicing the mesh model will left the smooth plane, which could induce the ambiguity when observing one object from a certain view, as a result making the self-occluded task to be more challenging.
% 4. The partial-to-partial task test with limited rotation range, to be specific, $[0, 45^{\circ}]$. However, in the real scene dataset the rotation range is wider than this, which is full rotation range. 

% 5. The last but not the least, the model which train with partial-to-partial augmentation cannot be directly used to solve self-occluded task.

% Comparing with the traditional RGB or RGB-D based 6D pose estimation task:

% 1. Traditional 6D pose estimation task focus on the known objects, but our task focus on generalization to unseen objects. In the traditional 6D pose task, the training and testing objects are the same, but in our task, the testing models are different from training models. This setting is non-trivial. 
% Since the XXX, XXX assume that the network could acquire enough knowledge about how to estimate the target object in the fixed coordinate reference system, thus in the training and testing process only takes the RGB or RGB-D images and predicts the 3D coordinates of the corner of the bounding box of object in the object coordinate system, like in the paper BB8. Then using PnP to get the final estimation of the pose. As for the RGB-D method, they using ICP for the final refinement. 
% In this case, if two objects' appearance are similar, but been placed in different direction in the reference system, the network could be confused. However, in our task, since we take both source and target pointcloud, thus this problem could be resolved. This setting makes our task is suitable for the unseen object pose estimation, whereas the traditional task setting are not.

% 2. The traditional 6D pose estimation task use the real scene data for fine-tuning, as in the paper CosyPose, but our task only use the object's mesh model. In the traditional setting, they use synthetic data for pre-training and fine-tune the model on both real and synthetic images or just real images. In our setting, we only take the synthetic mesh model as input, and evaluate our algorithm on the real scene data. Not mention our task also have to generalize to the unseen objects, the arduousness of our task is self-evident.

% 3. Our method is the first depth-based learning method on the unseen object 6D pose estimation task.

% 4. The real scene data is limited, thus pose a negative effect in the training process. However, with the propose viewpoint rendering augmentation, we can have infinity training sample, this problem can be fixed. \zd{From the experiment we show that the model trained with our viewpoint rendering augmentation is even better than using the real scene data.}

% \subsection{Viewpoint Rendering Augmentation}

% 1. Normalize the model.

% To introduce the core work of this paper, the viewpoint rendering augmentation, we need to get an idea about the estimating the 6D pose of the object of interest first. To this end, let $\bX \in \mathbb{R}^{M \times 3}$ and $\bY \in \mathbb{R}^{N \times 3}$ be two sets of 3D points sampled from the same object surface. We typically refer to $\bX$ as the source point set and to $\bY$ as the target point set. 
% % We obtain the source point set $\bX$ by visible surface sampling strategy~\ref{visible_surface} instead of uniform sampling from the mesh model which used in the paper DCP, RPMNet\ZD{add more paper}.
% We obtain the source point set $\bX$ through uniform sampling from the mesh model.
% The target one $\bY$ is obtained from $I_{depth}$ and $I_{mask}$, assuming known camera intrinsic parameters. Registration then aims to find a rigid transformation $\bT$ that aligns $\bX$ to $\bY$. In this work, we focus on the case where the object is self-occluded. To be specific, we assume that each point in $\bY$ has a corresponding point in $\bX$, but not the opposite.

% \paragraph{Combine with OPRNet Backbone.}

% The OPRNet backbone consists of a DGCNN~\cite{Wang18b} followed by a Transformer~\cite{Vaswani17}. Specifically, the DGCNN takes a point set as input, constructs a k-NN graph from it, and then extracts point-wise features via standard convolutions on this graph, encoding diverse levels of context by max-pooling the local features and concatenating the resulting representations to the point-wise ones.
% Let $\bthx$, resp. $\bthy$, be the final feature matrix, i.e., one $P$-dimensional feature vector per 3D point, for $\bX$, resp. $\bY$. The transformer then learns a function $\phi : \mathbb{R}^{M\times P} \times \mathbb{R}^{N\times P} \rightarrow \mathbb{R}^{M\times P}$, that combines the information of the two point sets. Ultimately, this produces descriptor matrices $\bfx$, resp. $\bfy$, for $\bX$, resp. $\bY$, written as
% \begin{equation}
%     \bfx = \bthx + \phi(\bthx, \bthy), \;\;\;
%     \bfy = \bthy + \phi(\bthy, \bthx)\;.
% \end{equation}
% Given these matrices, the OPRNet forms a score map $\bS \in \mathbb{R}^{M\times N}$ by computing the similarity between each source-target pair of descriptors. That is, we compute the $(i,j)$-th element of $\bS$ as
% \begin{equation}
%     \bS_{i,j} = <\bfx_i, \bfy_j>, \;\;\forall (i, j) \in [1,M]\times [1,N]\;,
% \end{equation}
% where $<\cdot, \cdot>$ is the inner product, and $\bfx_i, \bfy_j \in \mathbb{R}^P$. To handle the outlier and noise caused mismatch, the OPRNet adopts the Optimal Transport Layer~\cite{}. Specifically, it extends the score matrix $\bS$ by one row and one column to form an augmented score matrix $\bbS$. The values at the newly-created positions in $\bbS$ are set to
% \begin{equation}
%     \bbS_{i, N + 1} = \bbS_{M + 1, j} = \bbS_{M + 1, N + 1} = \alpha,
% \end{equation}
% $\forall i \in [1, M], \;\forall j \in [1, N]$, where $\alpha \in \mathbb{R}$ is a fixed parameter, which set to be $0.01$ in practice. The values at the other indices directly come from $\bS$. Given the augmented score map $\bbS$, we aim to find a partial assignment $\bbP \in \mathbb{R}^{(M+1)\times (N+1)}$, defining correspondences between the two point sets, extended with the outlier bins.

% In OPRNet, the supervision is directly imposed on the output of the Optimal Transportation Layer.
% To this end, let $\bM \in \{0, 1\}^{M \times N}$ be the matrix of ground-truth correspondences, with a $1$ indicating a correspondence between a pair of points. Such correspondences can be estimated using the ground-truth transformation matrix. To build the ground-truth assignment matrix $\bM$, as introduced in the OPRNet paper, we transform $\bX$ using the ground-truth transformation $\bT$, giving us $\btX$. We then compute the pairwise Euclidean distance matrix between $\btX$ and $\bY$, which we threshold to $0.05$ to obtain a correspondence matrix $\bM \in \{0, 1\}$. OPRNet augments $\bM$ with an extra row and column acting as outlier bins to obtain $\bbM$. The points without any correspondence are treated as outliers, and the corresponding positions in $\bbM$ are set to one. This strategy does not guarantee a bipartite matching, which OPRNet addresses using a forward-backward check. We keep using the loss function which used in the OPRNet, to be specific, the loss function is expressed as the negative log-likelihood

% \begin{equation}
%     \mathcal{L}(\bP, \bbM) = \frac{- \sum\limits_{i =1}^{M+1}\sum\limits_{j = 1}^{N+1} (\log \bP_{i,j})\bbM_{i, j}}{\sum\limits_{i = 1}^{M+1}\sum\limits_{j = 1}^{N+1} \bbM_{i, j}}\;,
%     \label{eq:nll}
% \end{equation}

% where $\bP$ is the output of the Optimal Transport Layer, and where the denominator normalizes the loss value so that different training samples containing different number of correspondences have the same influence in the overall empirical risk.

% \paragraph{Combine with IDAM Backbone.}

% We implement the viewpoint rendering augmentation using Pytorch3D. We generate scenes that contain individual object without background.

% \paragraph{Comparing to the Pointcloud Slicing Method.}


% \paragraph{Comparing to the real scene data.}


% \subsection{Visible Surface Sampling}
% \label{visible_surface}

% Some of the synthetic mesh models used in the training process have the inner structure, such as the seats in the car as shown in the Fig.\ZD{add the figure}. In this case, if we uniform sampling from the mesh model, the pointcloud of the inner structure will never found the corresponding point in the target point cloud. Thus here we introduce the visible surface sampling strategy, which sampling the points from the mesh model's visible surface. To be specific, we put the camera at the same place and rotating the object to 16 different angle. In this process we render the object's depth map and turn it back to the pointcloud by using camera parameter. We combine these 16 pointclouds to get final surface sampling pointcloud.

% And we found this module is very important when asymmetrical object augmentation is enable. 


% \subsection{Asymmetrical Object Augmentation}

% The symmetrical object been observed from different viewpoint can have same appearance. In the training process, the network takes the same input, but the loss is different. This ambiguity will interrupt the training and testing performance of the network.\ZD{Here we can use a comparison experiment to justify this statement. 500 asymmetrical object and 500 symmetrical object for training and evaluate on the asymmetrical clear dataset.}

% To eliminate the ambiguity in the training process bring by the symmetrical object, we introduce the asymmetrical object augmentation. To be specific, we add a sphere and a octahedron to merge with the object mesh model which its center be placed at the surface of the object. As shown in the figure, the octahedron and the sphere have been placed at the different place of the cup, thus make the symmetrical object asymmetrical. To be noticed, when merging two objects, if still sampling from the mesh model, the overlapping area which is hiding behind the surface also will be sampled. These points also cannot find the corresponding point in the target point cloud, which will make overlapping ratio lower. In this case, the use of 
% asymmetrical augmentation will not only fail to improve performance, but will further reduce performance.

==> tex/methodology_saved.tex <==
\section{Methodology}
\subsection{Problem Formulation}
Let us now introduce our approach to object-level 3D registration.
We consider the problem of partial-to-partial registration between two point clouds $\bX = \{\bx_1, \cdots, \bx_M\}$ and $\bY = \{\by_1, \cdots, \by_N\}$, which are two sets of 3D points sampled from the same object surface, with $\bx_i, \by_j \in \mathbb{R}^3$. We typically refer to $\bX$ as the source point set and to $\bY$ as the target point set. We obtain the source point set $\bX$ by uniform sampling from the mesh model, and the target one $\bY$ from a depth map $I_{depth}$ acquired by a depth sensor, assuming known camera intrinsic parameters. Our goal is to estimate the rotation matrix $\bR\in SO(3)$ and translation vector $\bt \in \mathbb{R}^{3}$ that align $\bX$ and $\bY$. The transformation $\bR, \bt$ can be estimated by solving
\begin{equation}
    \min_{\bR,\bt} = \sum_{\bx \in \bX_s} \norm{\bR\bx + \bt - \bQ(\bx)}^{2}_{2},
\label{eq:trans}
\end{equation}
where $\bQ:\bX_s\rightarrow\bY_s$ denotes the function that returns the best matches from set $\bX_s$ to set $\bY_s$, $\bX_s$ and $\bY_s$ the selected inlier point sets.
Given the matches, Eq.~\ref{eq:trans} can be solved via SVD~\cite{XX}. The challenging task therefore is to estimate the matching function $\bQ$, with only $\bX$ and $\bY$ as input.
% Registration then aims to find a rigid transformation $\bT$ that aligns $\bX$ to $\bY$.

\subsection{Method Overview}

Following the state-of-the-art 3D registration networks, our method is composed of two modules: the feature extraction module and the point matching module. The feature extraction module, denoted by $\Theta(\cdot,\cdot)$ takes two point set as input, and output the feature matrix, $\bthx$, resp. $\bthy$, i.e., one $P$-dimensional feature vector per 3D point, for $\bX$, resp. $\bY$. Then two feature matrices be passed to a transformer.
% The proposed network takes a point set as input, constructs a k-NN graph from it, and then extracts point-wise features via standard convolutions on this graph, encoding diverse levels of context by max-pooling the local features and concatenating the resulting representations to the point-wise ones.
The transformer then learns a function $\phi : \mathbb{R}^{M\times P} \times \mathbb{R}^{N\times P} \rightarrow \mathbb{R}^{M\times P}$, that combines the information of the two point sets. Ultimately, this produces descriptor matrices $\bfx$, resp. $\bfy$, for $\bX$, resp. $\bY$, written as
\begin{equation}
    \bfx = \bthx + \phi(\bthx, \bthy), \;\;\;
    \bfy = \bthy + \phi(\bthy, \bthx)\;.
\end{equation}

Given these matrices, we then form a score map $\bS \in \mathbb{R}^{M\times N}$ by computing the similarity between each source-target pair of descriptors. That is, we compute the $(i,j)$-th element of $\bS$ as
\begin{equation}
    \bS_{i,j} = <\bfx_i, \bfy_j>, \;\;\forall (i, j) \in [1,M]\times [1,N]\;,
\end{equation}
where $<\cdot, \cdot>$ is the inner product, and $\bfx_i, \bfy_j \in \mathbb{R}^P$. Then this matrix will be given to point matching module, Sinkhorn layer as in paper~\cite{}, this layer will find the best matches between two point sets and reject outlier points.

Our main contribution is in feature extraction network $\Theta(\cdot,\cdot)$, where we propose the construction of match normalization at each layer of $\Theta(\cdot,\cdot)$, as shown in the Figure XXX. Different from DCP, where the feature extraction network DGCNN treat the source and target point cloud separately, we use the match normalization to enforce the source and target point under the same scale normalization.

\subsubsection{Match Normalization}

% Our network based on the standard DGCNN network. The DGCNN takes the point set as input and using kNN to construct the graph. Then using a PointNet alike operation, using convolutional layer instead of MLP operate on the graph. At each layer, the convolutional layer will output a different graph feature. Before go through the next convolutional layer, the output graph feature will be normalized by Batch Normalization followed by ReLU. The DGCNN also keep the output graph of each in order to prepare for the final feature aggregation, which combines the local feature and global feature.\ZD{This part will be extended with symbols and formulas.}
PointNet~\cite{} a pioneer in the direction of learning-based point clouds feature extraction network. Most learning-based point registration method~\cite{} draw inspiration from this architecture. These feature extraction networks use a convolutional layer or MLP operates on a graph or the raw point set. Before the output feature by each layer go through the next layer, the output feature will be normalized by Batch Normalization followed by ReLU.
Then these the normalized features of each layer go though an additional network to aggregate the global feature, which is then be concatenated to the pointwise feature, to get the local and global information both.

Batch Normalization here be used to normalize the output of each layer which aims to smooth the distribution in order to speed up the training. Batch normalization assumes that every sample follows the same global statistics, thus normalizes the input over a mini-batch.
The object in the synthetic dataset perfectly match the Batch Normalization's assumption for it's clean, almost share the same size and sampled transformation in a small range, thus usually follow the similar distribution.
However, the objects in the real world and captured by the depth sensor are noisy, a variety of size and large range of transformation, thus make this assumption not always true. 
In this challenging scenario, subtracting and dividing by fixed scalar values for all the sample within one batch becomes the main reason cause the inferior performance. 
To solve this problem we introduce our Match Normalization. The central idea between the Match Normalization is forcing the two point set have the similar distribution, specifically, by centralizing the two point separately but scaling the source and target point set with the same parameter. Thus when feed them to the Batch Normalization this assumption will hold. To speed up training, we keep the Batch Normalization and put it after the Match Normalization, as shown in the Figure XXX.\ZD{Here would be illustration figure of the network architecture.}

Here we describe the formulation of the Match Normalization, let $\bo_{x}$ and $\bo_{y}$ be the output of layer $l$ when processing the $\bX$ and $\bY$ point set respectively. We take the normalized version of $\bo$ to be:
\ZD{going to modify this part to min-max format}
\begin{equation}
\begin{aligned}
    k_{share} = maximum\{|\bo_{x1}|, |\bo_{x2}|, |\bo_{xm}|\},\\
    \bho_{xi} = \frac{1}{k_{share}}(\bo_{xi} - \mu_{x}), \:\:\: \bho_{yi} = \frac{1}{k_{share}}(\bo_{yi} - \mu_{y}),
\end{aligned}
\end{equation}
where $\mu = \frac{1}{N}\sum^{N}_{i=1}\bo_i$ is calculated for $\bo_{x}$ and $\bo_{y}$ respectively, but scale $k_{share}$ is a shared parameter between the corresponding source and target point set. The goal is to normalize the point set pair set using the same scale. If we simply using the Match Normalization separately for the source and target point set, it has one fairly significant downside: it cannot handle outliers very well. The present of the outlier will squishes the rest points, thus the difference between the rest point would be small. Since the point in the source point set has stable scale, for it is sampled from the surface of the object's mesh model. And the source and target point set are should be geometrically similar, thus we use the same parameters in the network layer to normalise target point cloud set. This simple operation makes the source and target point set feature distribution shape aligned, which making the corresponding points in the two point sets more similar.

The Match Normalization is performed on the each pair of point set instance within a mini-batch, to make sure the pair of point set feature follow a similar distribution. By contrast, the Batch Normalization normalized the input of each layer over a mini-batch. These two normalization operates on the different dimension but the same goal is to make the mini-batch follows a consistent distribution during the training process. The consistent distribution properties aid the network generalization, such as having the same distribution between the training and test data, apply to the training of the network as well. And in the experiment, we do apply this combination to the design of the network. As shown in Fig.XXX\ZD{the figure of the network architecture.} XXX description of the network architecture.

\subsubsection{Hard Selection Sinkhorn}

Inspired by the previous works~\cite{}, we choose to use Sinkhorn layer to handle the partial-to-partial matching case. Specifically, we extend the score matrix $\bS$ by one row and one column to form an augmented score matrix $\bbS$. The values at the newly-created positions in $\bbS$ are set to
\begin{equation}
    \bbS_{i, N + 1} = \bbS_{M + 1, j} = \bbS_{M + 1, N + 1} = \alpha,
\end{equation}
$\forall i \in [1, M], \;\forall j \in [1, N]$, where $\alpha \in \mathbb{R}$ is a fixed parameter, which set to be $1$ in practice. The values at the other indices directly come from $\bS$. Given the augmented score map $\bbS$, we aim to find a partial assignment $\bbP \in \mathbb{R}^{(M+1)\times (N+1)}$, defining correspondences between the two point sets, extended with the outlier bins. Let $\bU (\ba, \bb)$ be the set of probability matrices defined as
\begin{equation}
    \left\{\bbP \in \mathbb{R}_{+}^{(M+1)\times (N+1)}: \bbP \mathbbm{1}_{M+1} = \ba \: \text{and}\: \bbP^{\top} \mathbbm{1}_{N+1} = \bb \right\}\;,
\end{equation}
where $\ba = [\mathbbm{1}_{M}^{\top}, N]^{\top}$, and $\bb = [\mathbbm{1}_{N}^{\top}, M]^{\top}$, with $\mathbbm{1}_{M} = [1, 1, ..., 1]^{\top}\in \mathbb{R}^{M}$. Then, from the optimal transport theory~\cite{Peyre19,Cuturi13}, an assignment probability matrix $\bbP$ can be obtained by solving
\begin{equation}
    \min_{\bbP \in \bU (\ba, \bb)} \langle \bbS, \bbP \rangle - \lambda E(\bbP)\;,
\label{entropy_func}
\end{equation}
where $\langle\cdot,\cdot\rangle$ is the Frobenius dot product and $E(\cdot)$ is an entropy regularization term defined as $E(\bbP) = - \displaystyle\sum_{i, j} \bbP_{i, j} \left(\log(\bbP_{i, j}) - 1\right)$. In practice, this optimization problem can be solved by using the log-domain Sinkhorn algorithm, where the matrix operator $logsumexp(\bA) = log(exp(\bA_{1,1}) + ... + exp(\bA_{i,j}) + ... + exp(\bA_{M,N}))$. Since all operations performed by this algorithm are differentiable, the training errors can be backpropagated to the rest of the network. We then still use the negative log-likelihood of Eq.~\ref{eq:nll} as loss function, but replacing $\bM$ with $\bbM$, which contains an extra row and column acting as outlier bins.

\subsubsection{Loss Function}

Instead, we impose direct supervision on the output of the Sinkhorn layer. To this end, let $\bM \in \{0, 1\}^{M \times N}$ be the matrix of ground-truth correspondences, with a $1$ indicating a correspondence between a pair of points. 
% Such correspondences can be estimated using the ground-truth transformation matrix,  
To build the ground-truth assignment matrix $\bM$, we transform $\bX$ using the ground-truth transformation $\bT$, giving us $\btX$. We then compute the pairwise Euclidean distance matrix between $\btX$ and $\bY$, which we threshold to obtain a correspondence matrix $\bM \in \{0, 1\}$. We augment $\bM$ with an extra row and column acting as outlier bins to obtain $\bbM$. The points without any correspondence are treated as outliers, and the corresponding positions in $\bbM$ are set to one. This strategy does not guarantee a bipartite matching, which we address using a forward-backward check.

We then express our loss function as the negative log-likelihood
\begin{equation}
    \mathcal{L}(\bP, \bM) = \frac{- \sum\limits_{i =1}^{M}\sum\limits_{j = 1}^{N} (\log \bP_{i,j})\bM_{i, j}}{\sum\limits_{i = 1}^{M}\sum\limits_{j = 1}^{N} \bM_{i, j}}\;,
    \label{eq:nll}
\end{equation}
where $\bP$ is the output of the Sinkhorn layer, and where the denominator normalizes the loss value so that different training samples containing different number of correspondences have the same influence in the overall empirical risk.

